Policy Synthesis for Switched Linear Systems with Markov Decision Process Switching

We study the synthesis of mode switching protocols for a class of discrete-time switched linear systems in which the mode jumps are governed by Markov decision processes (MDPs). We call such systems MDP-JLS for brevity. Each state of the MDP corresponds to a mode in the switched system. The probabilistic state transitions in the MDP represent the mode transitions. We focus on finding a policy that selects the switching actions at each mode such that the switched system that follows these actions is guaranteed to be stable. Given a policy in the MDP, the considered MDP-JLS reduces to a Markov jump linear system (MJLS). {We consider both mean-square stability and stability with probability one. For mean-square stability, we leverage existing stability conditions for MJLSs and propose efficient semidefinite programming formulations to find a stabilizing policy in the MDP. For stability with probability one, we derive new sufficient conditions and compute a stabilizing policy using linear programming. We also extend the policy synthesis results to MDP-JLS with uncertain mode transition probabilities.

==> modeEvolution.tex <==
% This file was created by tikzplotlib v0.8.2.
\begin{figure}
    \centering
    
\begin{tikzpicture}[scale=0.9]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=2 by 2,vertical sep=1.5cm},width=5cm,height=4cm]
\nextgroupplot[
tick align=outside,
tick pos=both,
title={SDP approximation},
x grid style={lightgray!92.02614379084967!black},
%xlabel={iterations},
xmajorgrids,
xmin=-2.45, xmax=51.45,
xtick style={color=black},
xtick={0,10,20,30,40,50},
%xticklabels={−20,0,20,40,60,,,},
y grid style={lightgray!92.02614379084967!black},
ylabel={System modes},
ymajorgrids,
ymin=-0.1, ymax=2.1,
ytick={0,1,2},
ytick style={color=black}
]
\addplot [semithick, color0, const plot mark right]
table {%
0 0
1 2
2 0
3 0
4 1
5 2
6 2
7 0
8 1
9 0
10 1
11 1
12 0
13 0
14 1
15 1
16 0
17 0
18 0
19 1
20 0
21 1
22 0
23 2
24 2
25 2
26 2
27 2
28 2
29 0
30 0
31 1
32 1
33 0
34 1
35 1
36 0
37 1
38 0
39 1
40 0
41 0
42 0
43 0
44 0
45 0
46 1
47 1
48 2
49 0
};

\nextgroupplot[
tick align=outside,
tick pos=both,
title={CD solution},
x grid style={lightgray!92.02614379084967!black},
%xlabel={iterations},
xmajorgrids,
xmin=-2.45, xmax=51.45,
xtick style={color=black},
xtick={0,10,20,30,40,50},
%xticklabels={−20,0,20,40,60,,,},
y grid style={lightgray!92.02614379084967!black},
ymajorgrids,
ymin=-0.1, ymax=2.1,
ytick={0,1,2},
ytick style={color=black}
]
\addplot [semithick, color0, const plot mark right]
table {%
0 0
1 0
2 0
3 0
4 1
5 1
6 1
7 1
8 1
9 1
10 1
11 1
12 1
13 1
14 1
15 1
16 1
17 1
18 1
19 1
20 1
21 0
22 0
23 0
24 0
25 1
26 1
27 1
28 1
29 1
30 1
31 0
32 0
33 0
34 1
35 1
36 1
37 1
38 1
39 1
40 1
41 1
42 1
43 1
44 1
45 1
46 1
47 1
48 1
49 1
};

\nextgroupplot[
tick align=outside,
tick pos=both,
title={Mode independent LP},
x grid style={lightgray!92.02614379084967!black},
xlabel={Number of time-steps},
xmajorgrids,
xmin=-2.45, xmax=51.45,
xtick style={color=black},
xtick={0,10,20,30,40,50},
%xticklabels={−20,0,20,40,60,,,},
y grid style={lightgray!92.02614379084967!black},
ylabel={System modes},
ymajorgrids,
ymin=-0.1, ymax=2.1,
ytick={0,1,2},
ytick style={color=black}
]
\addplot [semithick, color0, const plot mark right]
table {%
0 0
1 0
2 2
3 0
4 1
5 0
6 0
7 0
8 0
9 0
10 0
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 1
31 1
32 0
33 0
34 0
35 0
36 1
37 1
38 1
39 0
40 0
41 1
42 1
43 1
44 1
45 1
46 1
47 1
48 1
49 1
};

\nextgroupplot[
tick align=outside,
tick pos=both,
title={Mode dependent LP},
x grid style={lightgray!92.02614379084967!black},
xlabel={Number of time-steps},
xmajorgrids,
xmin=-2.45, xmax=51.45,
xtick style={color=black},
xtick={0,10,20,30,40,50,60},
%xticklabels={−20,0,20,40,60,,,},
y grid style={lightgray!92.02614379084967!black},
ymajorgrids,
ymin=-0.1, ymax=2.1,
ytick={0,1,2},
ytick style={color=black}
]
\addplot [semithick, color0, const plot mark right]
table {%
0 0
1 0
2 2
3 2
4 2
5 0
6 1
7 1
8 1
9 1
10 1
11 1
12 0
13 0
14 1
15 2
16 2
17 0
18 0
19 0
20 1
21 0
22 1
23 0
24 0
25 1
26 0
27 1
28 0
29 0
30 1
31 0
32 1
33 0
34 0
35 0
36 1
37 1
38 0
39 2
40 2
41 0
42 2
43 0
44 2
45 0
46 1
47 1
48 0
49 1
};
\end{groupplot}

\end{tikzpicture}

    \caption{Mode transition of the system w.r.t. the number of time steps for policies generated from the four methods explained in this sequel.}
    \label{fig:nummode}
\end{figure}

==> stateEvolution1.tex <==
% This file was created by tikzplotlib v0.8.2.
\begin{figure}
    \centering
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

%width, height represents the size of the figure, vertical sep does the spacing between figure
\begin{groupplot}[group style={group size=2 by 2,vertical sep=2cm},width=5cm,height=4cm]
\nextgroupplot[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=both,
title={SDP approximation},
x grid style={lightgray!92.02614379084967!black},
%xlabel={iterations},
xmajorgrids,
xmin=-2.45, xmax=51.45,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
ylabel={Current value of state},
ymajorgrids,
ymin=1e-07, ymax=2.62492381051258,
ytick style={color=black},
ytick={-1,0,1,2,3},
yticklabels={−0.5,0.0,0.5,1.0,1.5}
]
\addplot [semithick, color0]
table {%
0 2.5
1 1.8
2 1.4025
3 1.2
4 1.08
5 0.96310875
6 0.859126375
7 0.7678518125
8 0.68509094875
9 0.61084794575
10 0.5328985123875
11 0.47960866114875
12 0.431647795033875
13 0.388483015530488
14 0.363054867050124
15 0.325422705685324
16 0.290918063576562
17 0.259719640295179
18 0.231561359633196
19 0.206264309810129
20 0.183595126737637
21 0.163327337506044
22 0.141718475872614
23 0.125662215201347
24 0.112043801130675
25 0.0997143696664138
26 0.0867989112206015
27 0.0748291086104093
28 0.0673461977493684
29 0.0601393982954583
30 0.0541254584659124
31 0.0486484459082294
32 0.0433954391552927
33 0.038776159351023
34 0.0339670704166096
35 0.0305703633749487
36 0.0272169026254669
37 0.0244952123629202
38 0.0220456911266282
39 0.0198411220139653
40 0.0187657223642691
41 0.0167374038012258
42 0.0150636634211032
43 0.0135351629152943
44 0.0121816466237649
45 0.010979287208774
46 0.00962687357208328
47 0.00866418621487496
48 0.00777466205603418
49 0.00699719585043076
};
\addlegendentry{X0}
\addplot [semithick, color1]
table {%
0 0.75
1 1.75
2 1.4375
3 1.29875
4 1.2823625
5 1.06518125
6 0.94516575
7 0.849524625
8 0.7543079625
9 0.670264810875
10 0.5827402144375
11 0.574497571449375
12 0.563959543759532
13 0.551476372807149
14 0.410849937318296
15 0.36598050780482
16 0.323722408408075
17 0.286945847924232
18 0.254233298658665
19 0.22539117813955
20 0.199875923018618
21 0.177309903204688
22 0.154533791034667
23 0.134859473484997
24 0.122240704105392
25 0.108457924969649
26 0.0948076672011289
27 0.0813157254070482
28 0.0802807725151234
29 0.0665592316177462
30 0.0656663694598716
31 0.0540180139474262
32 0.0477815487054996
33 0.0428739816216323
34 0.0372237043521712
35 0.036708640743252
36 0.0300763226883038
37 0.0296725995133431
38 0.0291455589416407
39 0.0285142882209857
40 0.0213556429334658
41 0.0185128118199084
42 0.018263694974412
43 0.0150267731482722
44 0.0148266176380916
45 0.0122079887027409
46 0.0105551456824185
47 0.0104192034298273
48 0.00862567698595281
49 0.00851070689784037
};
\addlegendentry{X1}
\addplot [semithick, color2]
table {%
0 1
1 1.075
2 1.195
3 1.06975
4 1.0503625
5 0.88639375
6 0.805507125
7 0.7080949875
8 0.6277518675
9 0.554632483125
10 0.467729056725
11 0.458625927953125
12 0.446607873437531
13 0.433216859106105
14 0.349788120452246
15 0.305798990283028
16 0.269851894339298
17 0.237856473970529
18 0.210152221035717
19 0.185836788895339
20 0.164512361159346
21 0.14574024456329
22 0.122874345032559
23 0.115140289695977
24 0.100793287618737
25 0.089900964735844
26 0.0758325395934948
27 0.0671032843651922
28 0.0657722654861241
29 0.0551218217825418
30 0.0539105694289399
31 0.0447668242870911
32 0.0405980802678892
33 0.0356712493533193
34 0.0301790661093499
35 0.0295822820016589
36 0.0248612792519265
37 0.0243091752297181
38 0.0236200123435549
39 0.0228701638529663
40 0.0182599012755478
41 0.015305882928663
42 0.0149898828754412
43 0.0125152731776368
44 0.0122343307817169
45 0.0101310041560629
46 0.00876457274092994
47 0.00858716775703067
48 0.00717729015362252
49 0.00701782746658569
};
\addlegendentry{X2}
\addplot [semithick, color3]
table {%
0 1.5
1 0.8
2 0.535
3 0.453
4 0.2718
5 0.3187925
6 0.248035625
7 0.204568525
8 0.17309376125
9 0.149322067375
10 0.170655323575
11 0.102393194145
12 0.061435916487
13 0.0368615498922
14 0.101387991778101
15 0.0856728079342751
16 0.0734163029954403
17 0.06369334093165
18 0.0556323178628779
19 0.0488313810350107
20 0.0429993694070392
21 0.0379509208194543
22 0.0443284172404397
23 0.0344516431234757
24 0.0287398505313356
25 0.0244492540275415
26 0.0277598945581854
27 0.0262704657419731
28 0.0157622794451839
29 0.0194593648752984
30 0.011675618925179
31 0.0154523614558596
32 0.0122028631566389
33 0.0101612396051084
34 0.0111987457127072
35 0.00671924742762433
36 0.0086041553713815
37 0.0051624932228289
38 0.00309749593369734
39 0.0018584975602184
40 0.00531743179468062
41 0.0057789529729818
42 0.00346737178378908
43 0.00438492528860388
44 0.00263095517316233
45 0.00349924822560832
46 0.00342590012145592
47 0.00205554007287355
48 0.00253964958055555
49 0.00152378974833333
};
\addlegendentry{X3}

\nextgroupplot[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=both,
title={CD solution},
x grid style={lightgray!92.02614379084967!black},
%xlabel={iterations},
xmajorgrids,
xmin=-2.45, xmax=51.45,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
%ylabel={states},
ymajorgrids,
ymin=-0.124949156449467, ymax=2.62499757887855,
ytick style={color=black},
ytick={-1,0,1,2,3},
yticklabels={−0.5,0.0,0.5,1.0,1.5}
]
\addplot [semithick, color0]
table {%
0 2.5
1 1.8
2 1.4025
3 1.2
4 1.040925
5 0.9280825
6 0.81984975
7 0.714909375
8 0.62568423
9 0.563115807
10 0.5068042263
11 0.4603889115975
12 0.416739035522438
13 0.365427786873
14 0.319150671539199
15 0.279210735609734
16 0.251289662048761
17 0.226160695843885
18 0.209262583655279
19 0.187272663281635
20 0.165421466781357
21 0.143987709268723
22 0.125728376462816
23 0.110031953996301
24 0.0964796732007816
25 0.0868317058807034
26 0.0781485352926331
27 0.0703336817633698
28 0.0633003135870328
29 0.0569702822283295
30 0.0512732540054966
31 0.0461459286049469
32 0.0415313357444522
33 0.037378202170007
34 0.0336403819530063
35 0.0302763437577057
36 0.0272487093819351
37 0.0245238384437416
38 0.0253152868374017
39 0.0292494921972019
40 0.0281906905792195
41 0.025468602962164
42 0.0229217426659476
43 0.0206295683993529
44 0.0185666115594176
45 0.0167099504034758
46 0.0150389553631282
47 0.0135350598268154
48 0.0121815538441339
49 0.0109633984597205
};
\addlegendentry{X0}
\addplot [semithick, color1]
table {%
0 0.75
1 1.75
2 1.4375
3 1.29875
4 1.134875
5 1.015965
6 0.902375
7 0.78159075
8 0.6853523625
9 0.67692610425
10 0.66563851915625
11 0.55989662450875
12 0.464370603405313
13 0.400676793693781
14 0.349203892462166
15 0.305775890246624
16 0.302023979995124
17 0.296993937266661
18 0.235690624836855
19 0.209229881851015
20 0.182066112994777
21 0.157268782057193
22 0.137553439470333
23 0.120522401762426
24 0.105783478336486
25 0.104496447524247
26 0.102766134107031
27 0.100653772408886
28 0.098226504479802
29 0.0955498073046096
30 0.0926837630575419
31 0.0896815114711141
32 0.0865889063986467
33 0.0834448056564034
34 0.0802816650556772
35 0.0771262506073083
36 0.0740003670054765
37 0.070921549511325
38 0.0500225418474297
39 0.0360915102433024
40 0.0323597382000982
41 0.028352326313997
42 0.0280225794031831
43 0.0275721550921015
44 0.027017255696667
45 0.0263759106565015
46 0.0256658245902677
47 0.0249033080375311
48 0.0241028240890194
49 0.0232768759067912
};
\addlegendentry{X1}
\addplot [semithick, color2]
table {%
0 1
1 1.075
2 1.195
3 1.06975
4 0.953425
5 0.8766675
6 0.74333175
7 0.65579535
8 0.57649533
9 0.564984699625
10 0.549455305575
11 0.468352295213125
12 0.384614551865125
13 0.332979998051331
14 0.292401108954049
15 0.257302839853502
16 0.252157443372239
17 0.245220553829825
18 0.198625963574121
19 0.176859562707919
20 0.149116097333029
21 0.131119169671943
22 0.115316427062036
23 0.101535002676671
24 0.0893466672274211
25 0.0875549208234716
26 0.0851364989585179
27 0.0824285044727263
28 0.0796187518687231
29 0.076808447439536
30 0.0740492403810299
31 0.0713649928879343
32 0.0687644622079747
33 0.0662485971282765
34 0.0638146591909691
35 0.0614584854202762
36 0.059175674745986
37 0.0569621608240845
38 0.046867733649203
39 0.0354699842029945
40 0.0285139620487744
41 0.0246411114495533
42 0.0241149299187865
43 0.0234167538761602
44 0.0226409990306052
45 0.0218401495848516
46 0.0210423627626756
47 0.0202618772780119
48 0.0195051306893416
49 0.0187743242672109
};
\addlegendentry{X2}
\addplot [semithick, color3]
table {%
0 1.5
1 0.8
2 0.535
3 0.453
4 0.39515
5 0.2929175
6 0.2925005
7 0.26566655
8 0.23742569
9 0.142455414
10 0.0854732484
11 0.0976821547575
12 0.132743320945625
13 0.130020238751275
14 0.118604095110776
15 0.10592185983512
16 0.0635531159010722
17 0.0381318695406433
18 0.0642968585822224
19 0.0520110256485233
20 0.056176322800993
21 0.052293748587003
22 0.0471413333691897
23 0.041919818760083
24 0.0370749280393674
25 0.0222449568236204
26 0.0133469740941723
27 0.00800818445650336
28 0.00480491067390202
29 0.00288294640434121
30 0.00172976784260473
31 0.00103786070556284
32 0.000622716423337701
33 0.000373629854002621
34 0.000224177912401572
35 0.000134506747440943
36 8.07040484645661e-05
37 4.84224290787396e-05
38 0.00572042729694782
39 0.0116617176486197
40 0.0117586839000468
41 0.0104062659697736
42 0.00624375958186416
43 0.00374625574911849
44 0.0022477534494711
45 0.00134865206968266
46 0.000809191241809594
47 0.000485514745085757
48 0.000291308847051454
49 0.000174785308230872
};
\addlegendentry{X3}

\nextgroupplot[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=both,
title={Mode independent LP},
x grid style={lightgray!92.02614379084967!black},
xlabel={Number of time-step},
xmajorgrids,
xmin=-2.45, xmax=51.45,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
ylabel={Current value of state},
ymajorgrids,
ymin=-0.124968687782697, ymax=2.62499850894203,
ytick style={color=black},
ytick={-1,0,1,2,3},
yticklabels={−0.5,0.0,0.5,1.0,1.5}
]
\addplot [semithick, color0]
table {%
0 2.5
1 1.8
2 1.4025
3 1.2
4 1.040925
5 0.9105825
6 0.81952425
7 0.737982975
8 0.658790985
9 0.57542477025
10 0.517882293225
11 0.46491332142375
12 0.40778410005225
13 0.367005690047025
14 0.330305121042323
15 0.304627110631138
16 0.274164399568024
17 0.246747959611222
18 0.2220731636501
19 0.19986584728509
20 0.179879262556581
21 0.161891336300923
22 0.14570220267083
23 0.131131982403747
24 0.118018784163373
25 0.106216905747035
26 0.124933163712901
27 0.12266490658522
28 0.110333395205564
29 0.0980107553925108
30 0.0865005737616201
31 0.076199143981772
32 0.0670590719780214
33 0.0589887366348602
34 0.0518768791867845
35 0.0456164004611694
36 0.0401084727423555
37 0.035264147337017
38 0.0317377326033153
39 0.0285639593429838
40 0.0257075634086854
41 0.0231368070678169
42 0.0208231263610352
43 0.0187408137249317
44 0.0168667323524385
45 0.0151800591171947
46 0.0136620532054752
47 0.0122958478849277
48 0.0110662630964349
49 0.00995963678679141
};
\addlegendentry{X0}
\addplot [semithick, color1]
table {%
0 0.75
1 1.75
2 1.4375
3 1.29875
4 1.134875
5 0.997175
6 0.9850055
7 0.85467625
8 0.7289934875
9 0.62964579125
10 0.62167929935
11 0.51591438909375
12 0.447183506041875
13 0.441471415682194
14 0.433915211650617
15 0.342559290530735
16 0.337933178615563
17 0.331893398749868
18 0.324665258624949
19 0.316476455598742
20 0.3075401694767
21 0.298047414605244
22 0.288164567902903
23 0.278033680011031
24 0.267774182485986
25 0.257485200094502
26 0.155113486647984
27 0.141974929118916
28 0.122556538716663
29 0.108184561384736
30 0.095162245239778
31 0.0837482864221433
32 0.0736655479724829
33 0.0647850250690897
34 0.0569670969938775
35 0.0500888945085567
36 0.0440392543400078
37 0.0387193425238506
38 0.0382515690374848
39 0.0376212043081467
40 0.0368505752341051
41 0.0359642426288868
42 0.0349861950422519
43 0.0339384638403048
44 0.0328405456281766
45 0.0317092705070197
46 0.0305589050742915
47 0.0294013684531515
48 0.0282464925204895
49 0.0271022886023455
};
\addlegendentry{X1}
\addplot [semithick, color2]
table {%
0 1
1 1.075
2 1.195
3 1.06975
4 0.953425
5 0.8403775
6 0.82363575
7 0.720004
8 0.6005005975
9 0.52453697425
10 0.5139464849625
11 0.42945369066
12 0.372341104837875
13 0.364813060685831
14 0.354813460019148
15 0.287969232126888
16 0.280906360349197
17 0.272476035390132
18 0.263481293075658
19 0.254361341471568
20 0.245345978967685
21 0.236546558862753
22 0.228009175297541
23 0.219745427117413
24 0.211749932978912
25 0.204010067548933
26 0.159016694524931
27 0.122448170848106
28 0.106035727563909
29 0.0923137350870452
30 0.0809959990826666
31 0.0711319519631938
32 0.062510978160158
33 0.0549454573528947
34 0.0483009098303289
35 0.0424621082188461
36 0.0373302123053458
37 0.0328190679833675
38 0.0321581108848919
39 0.0312658677924781
40 0.0302669349551583
41 0.0292307264572601
42 0.0281946396845259
43 0.0271777497131144
44 0.0261888564807753
45 0.0252311732422808
46 0.0243050245203083
47 0.0234093703681347
48 0.0225426435816645
49 0.0217031889461339
};
\addlegendentry{X2}
\addplot [semithick, color3]
table {%
0 1.5
1 0.8
2 0.535
3 0.453
4 0.39515
5 0.348745
6 0.209247
7 0.186987075
8 0.21879563
9 0.2076183715
10 0.1245710229
11 0.1526177061525
12 0.146937820593
13 0.0881626923558
14 0.05289761541348
15 0.0921217381692215
16 0.0552730429015329
17 0.0331638257409198
18 0.0198982954445519
19 0.0119389772667311
20 0.00716338636003867
21 0.0042980318160232
22 0.00257881908961392
23 0.00154729145376835
24 0.000928374872261011
25 0.000557024923356607
26 0.0410248234791292
27 0.0482132682966378
28 0.0437749414882764
29 0.0387171221080923
30 0.0339495958606459
31 0.0297790381607917
32 0.0261380056569554
33 0.0229573978948138
34 0.0201720506285045
35 0.0177290022174676
36 0.0155840225307563
37 0.0136996514733717
38 0.00821979088402299
39 0.00493187453041379
40 0.00295912471824828
41 0.00177547483094897
42 0.00106528489856938
43 0.000639170939141628
44 0.000383502563484976
45 0.000230101538090986
46 0.000138060922854592
47 8.28365537127549e-05
48 4.9701932227653e-05
49 2.98211593365918e-05
};
\addlegendentry{X3}

\nextgroupplot[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=both,
title={Mode dependent LP},
x grid style={lightgray!92.02614379084967!black},
xlabel={Number of time-steps},
xmajorgrids,
xmin=-2.45, xmax=51.45,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
%ylabel={states},
ymajorgrids,
ymin=-0.124320926776577, ymax=2.62496766317984,
ytick style={color=black},
ytick={-1,0,1,2,3},
yticklabels={−0.5,0.0,0.5,1.0,1.5}
]
\addplot [semithick, color0]
table {%
0 2.5
1 1.8
2 1.4025
3 1.2
4 1.08
5 0.972
6 0.8901103125
7 0.78496550625
8 0.685401076875
9 0.61106310475
10 0.5464824078125
11 0.487855107371875
12 0.4276188328155
13 0.38485694953395
14 0.342499430230186
15 0.305276767180824
16 0.272641488596673
17 0.238541049223046
18 0.206563907297713
19 0.185907516567941
20 0.166374729313885
21 0.145728299125196
22 0.127269528004927
23 0.114542575204434
24 0.10307126129525
25 0.0924752295709336
26 0.081665264392817
27 0.0734987379535353
28 0.0656132653898765
29 0.057386288146767
30 0.0500389772736712
31 0.0437488446206491
32 0.0383302780516433
33 0.0336315852947482
34 0.0302684267652733
35 0.0273284992331307
36 0.0240434884266391
37 0.0216391395839752
38 0.0194745687271824
39 0.0171022907930878
40 0.0149550702507405
41 0.0130962622297972
42 0.0117866360068175
43 0.0106079724061358
44 0.00954717516552219
45 0.00859245764896997
46 0.00838875321551011
47 0.00758367069090504
48 0.00665930153539052
49 0.00583921409544107
};
\addlegendentry{X0}
\addplot [semithick, color1]
table {%
0 0.75
1 1.75
2 1.4375
3 1.29875
4 1.2823625
5 1.260644375
6 0.9975171875
7 0.8632206875
8 0.749852375
9 0.6693020143125
10 0.60533895435
11 0.538358418823125
12 0.468770501006563
13 0.462245475819244
14 0.378403908950002
15 0.334816725842433
16 0.300646749582803
17 0.261247671073407
18 0.225002654217998
19 0.222154719830455
20 0.18433745723917
21 0.159693133885051
22 0.139251730445613
23 0.137525354844499
24 0.119053849188745
25 0.104823250899991
26 0.0898711592025616
27 0.0886278634294097
28 0.0726060733396932
29 0.0628371808830068
30 0.0547051513827352
31 0.0478952523975795
32 0.0420093744424143
33 0.0368875031320919
34 0.0364395407930516
35 0.0304132853392478
36 0.0264082310944999
37 0.0260738722403809
38 0.0216380447533163
39 0.0187665336248886
40 0.0163739716880235
41 0.0143495685909585
42 0.0141739696312558
43 0.0139383443241243
44 0.0136510246812225
45 0.0133211226094927
46 0.00968502653469853
47 0.00844507454375334
48 0.00730700054686502
49 0.00640237272470652
};
\addlegendentry{X1}
\addplot [semithick, color2]
table {%
0 1
1 1.075
2 1.195
3 1.06975
4 1.0503625
5 1.023034375
6 0.8363310625
7 0.71473924375
8 0.6274224325
9 0.576319240125
10 0.50669181121875
11 0.44968589464125
12 0.37942166545125
13 0.371950868366053
14 0.312772229966754
15 0.284200748520139
16 0.249853853550141
17 0.21146425921295
18 0.186482713387431
19 0.182767397910399
20 0.153011538456218
21 0.132775161766031
22 0.116706420864018
23 0.114372011317029
24 0.100182205347334
25 0.0872670888341895
26 0.0732111385492683
27 0.0717134087258511
28 0.060061096376137
29 0.0520240146187033
30 0.0457515275214878
31 0.0402699042641796
32 0.0354447282125405
33 0.0311841741886292
34 0.0305581439132222
35 0.0254879629558691
36 0.0220857966799812
37 0.0216369499226574
38 0.0180584985225947
39 0.0156456525829592
40 0.0137440669311765
41 0.0120908957580657
42 0.0118487971130647
43 0.0115223233840756
44 0.011156832762327
45 0.0107775954204271
46 0.00850139587199658
47 0.00703033040282499
48 0.00614544391402252
49 0.00539201330974462
};
\addlegendentry{X2}
\addplot [semithick, color3]
table {%
0 1.5
1 0.8
2 0.535
3 0.453
4 0.2718
5 0.16308
6 0.269838875
7 0.2752017625
8 0.25302855375
9 0.189256520125
10 0.152260184075
11 0.126799273159375
12 0.140656888192
13 0.0843941329152
14 0.108147826839291
15 0.0853511364163207
16 0.0710956430601743
17 0.0784090279340978
18 0.073656463016229
19 0.0441938778097374
20 0.0542310307059749
21 0.0522947199736335
22 0.0474729203426595
23 0.0284837522055957
24 0.0256790772345008
25 0.0228577591519838
26 0.0265965214276314
27 0.0159579128565789
28 0.0207258468878018
29 0.0203025580303481
30 0.0185258261358799
31 0.0165606359586495
32 0.0146782352362957
33 0.0129602397370264
34 0.00777614384221584
35 0.00922208631953078
36 0.00878642711898614
37 0.00527185627139168
38 0.00643613249308815
39 0.00618615270175421
40 0.00560359159729353
41 0.00499025002515272
42 0.00299415001509163
43 0.00179649000905498
44 0.00107789400543299
45 0.000646736403259792
46 0.00241421364538934
47 0.00266596463255505
48 0.00247245193358702
49 0.00221806955623931
};
\addlegendentry{X3}
\end{groupplot}

\end{tikzpicture}
    \caption{Caption}
    \label{fig:numstate}
\end{figure}
